Cost-effective Selection of Pretraining Data: A Case Study of Pretraining BERT on Social Media

Recent studies on domain-specific BERT models show that effectiveness on downstream tasks can be improved when models are pretrained on in-domain data. Often, the pretraining data used in these models are selected based on their subject matter, e.g., biology or computer science. Given the range of applications using social media text, and its unique language variety, we pretrain two models on tweets and forum text respectively, and empirically demonstrate the effectiveness of these two resources. In addition, we investigate how similarity measures can be used to nominate in-domain pretraining data. We publicly release our pretrained models at https://bit.ly/35RpTf0.

==> src/table-vocab.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{r|c|c}
    \toprule
         & CoNLL 2003 & W-NUT 2016 \\
    \toprule
    \# tokens & 301,418 & 124,638 \\
    \# unique tokens & 30,289 & 21,443 \\
    \# tokens directly found in BERT vocab & 250,668 (83.1) & 91,788 (73.6) \\
    \# unique tokens directly found in BERT vocab & 11,574 (38.2) & 7,994 (37.2) \\
    \# sub-tokens after wordpiece tokenization & 404,004 & 211,810 \\
    Average sub-tokens per token & 1.34 & 1.69 \\
    \bottomrule
    \end{tabular}
    \caption{Comparison between CoNLL 2003 and W-NUT 2016, which are sampled from news articles and twitter, separately.~\label{table:news_vs_twitter}}
\end{table}
